Deterministic fabrication of GaAs-quantum-dot micropillar single-photon sources

This study investigates the performance of droplet-etched GaAs quantum dots (QDs) integrated into micropillar structures using a deterministic fabrication technique. We demonstrate a unity QD positioning yield across 74 devices and consistent device performance. Under p-shell excitation, the QD decay dynamics within the micropillars exhibit biexponential behavior, accompanied by intensity fluctuations limiting the source efficiency to < 4.5%. Charge stabilization via low-power above-band LED excitation effectively reduces these fluctuations, doubling the source efficiency to $\sim$ 9%. Moreover, we introduce suppression of radiation modes by introducing cylindrical rings theoretically predicted to boost the collection efficiency by a factor of 4. Experimentally, only a modest improvement is obtained, underscoring the influence of even minor fabrication imperfections for this advanced design. Our findings demonstrate the reliability of our deterministic fabrication approach in producing high-yield, uniform devices, while offering detailed insights into the influence of charge noise and complex relaxation dynamics on the performance.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
